Atmospheric NLTE-Models for the Spectroscopic Analysis of Blue Stars with Winds. II. Line-Blanketed Models

We present new or improved methods for calculating NLTE, line-blanketed model atmospheres for hot stars with winds (spectral types A to O), with particular emphasis on a fast performance. These methods have been implemented into a previous, more simple version of the model atmosphere code FASTWIND (Santolaya-Rey et al.1997) and allow to spectroscopically analyze rather large samples of massive stars in a reasonable time-scale, using state-of-the-art physics. We describe our (partly approximate) approach to solve the equations of statistical equilibrium for those elements which are primarily responsible for line-blocking and blanketing, as well as an approximate treatment of the line-blocking itself, which is based on a simple statistical approach using suitable means for line opacities and emissivities. Furthermore, we comment on our implementation of a consistent temperature structure. In the second part, we concentrate on a detailed comparison with results from those two codes which have been used in alternative spectroscopical investigations, namely CMFGEN (Hillier & Miller 1998) and WM-Basic (Pauldrach et al. 2001). All three codes predict almost identical temperature structures and fluxes for lambda > 400 A, whereas at lower wavelengths a number of discrepancies are found. Optical H/He lines as synthesized by FASTWIND are compared with results from CMFGEN, obtaining a remarkable coincidence, except for the HeI singlets in the temperature range between 36,000 to 41,000 K for dwarfs and between 31,000 to 35,000 K for supergiants, where CMFGEN predicts much weaker lines. Consequences due to these discrepancies are discussed.

==> plots/metaplot <==
#FIG 3.2
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 450 5400 2250 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 450 4500 2250 4500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 450 1350 2250 1350
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 2250 4500 2250
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 5400 4500 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 450 4500 2250 4500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 1350 4500 1350
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 1 2
	1 1 2.00 120.00 240.00
	 855 1350 855 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 2.00 120.00 240.00
	 1800 1350 1800 4500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 1 2
	1 1 2.00 120.00 240.00
	 3150 1350 3150 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 2.00 120.00 240.00
	 4050 1350 4050 2250
4 0 0 50 0 0 20 0.0000 4 135 240 2385 4590 m\001
4 0 0 50 0 0 20 0.0000 4 195 390 450 6345 m1\001
4 0 0 50 0 0 20 0.0000 4 135 240 4635 2340 m\001
4 0 0 50 0 0 20 0.0000 4 270 90 2430 1395 j\001
4 0 0 50 0 0 20 0.0000 4 195 150 2430 5490 1\001
4 0 0 50 0 0 20 0.0000 4 195 150 4680 5490 1\001
4 0 0 50 0 0 20 0.0000 4 270 90 4635 1395 j\001
4 0 0 50 0 0 20 0.0000 4 195 390 2700 6345 m2\001

